Representation Learning for Grounded Spatial Reasoning

The interpretation of spatial references is highly contextual, requiring joint inference over both language and the environment. We consider the task of spatial reasoning in a simulated environment, where an agent can act and receive rewards. The proposed model learns a representation of the world steered by instruction text. This design allows for precise alignment of local neighborhoods with corresponding verbalizations, while also handling global references in the instructions. We train our model with reinforcement learning using a variant of generalized value iteration. The model outperforms state-of-the-art approaches on several metrics, yielding a 45% reduction in goal localization error.

==> rl.tex <==
% \begin{table}[t]
% %   \footnotesize
%   \renewcommand\arraystretch{1.3}
%   \renewcommand\tabcolsep{0pt}
%   \begin{tabular*}{1\linewidth}{@{\extracolsep{\fill}}lcccc}
%         \toprule
%         & \multicolumn{2}{c}{Local} & \multicolumn{2}{c}{Global} \\
%         \cmidrule(lr){2-3}\cmidrule(lr){4-5}
%         & Quality & Distance
%         & Quality & Distance \\
%         \midrule
%         UVFA (text) & 0.56 & 4.71 & 0.62 & 6.28 \\
%         CNN + LSTM & 0.80 & 5.73 & 0.82 & 6.13 \\
%         Ours & \textbf{0.87} & \textbf{2.18} & \textbf{0.90} & \textbf{3.35} \\
%         \bottomrule
%   \end{tabular*}
%   \vspace{0.1cm}
%   \caption{RL generalization to new environments and instructions.}
%   \label{tbl:rl_eval}
% %   \vspace{-10pt}
% \end{table}

% \begin{table*}[t]
%   \renewcommand\arraystretch{1.3}
%   \renewcommand\tabcolsep{0pt}
%   \begin{tabular*}{1\linewidth}{@{\extracolsep{\fill}}lcccccc}
%         \toprule
%         & \multicolumn{3}{c}{Local} & \multicolumn{3}{c}{Global} \\
%         \cmidrule(lr){2-4}\cmidrule(lr){5-7}
%         & MSE & Policy Quality & Distance
%         & MSE & Policy Quality & Distance \\
%         \midrule
%         UVFA (pos) & 1.30 & 0.48 & 4.96 & 1.04 & 0.52 & 5.39 \\
%         UVFA (text) & 3.23 & 0.57 & 4.97 & 1.9 & 0.62 & 5.31 \\
%         CNN + LSTM & 0.42 & 0.86 & 4.08 & 0.43 & 0.83 & 4.18 \\
%         \midrule
%         No gradient & \textbf{0.25} & \textbf{0.92} & 2.39 & 0.61 & 0.87 & 5.15 \\
%         Ours & \textbf{0.25} & \textbf{0.92} & \textbf{2.34} & \textbf{0.41} & \textbf{0.89} & \textbf{3.81}  \\
%         \bottomrule
%   \end{tabular*}
%   \vspace{0.1cm}
%   \caption{Supervised results on the standard train-test split, requiring generalization over both instructions and environment configurations. Distance is the mean Manhattan distance from the actual goal to the predicted goal, determined by the position of the maximum value prediction.}
%   \label{tbl:analysis}
% %   \vspace{-10pt}
% \end{table*}

% \subsection{Results}
% We first investigate the ability of our model to learn via environment simulation alone. Fig~\ref{fig:learning_curves} shows the discounted reward achieved by our model as well as the two baselines for both instruction types. In both experiments, our model is the only one of the three to achieve an average nonnegative reward (0.88 for local instructions and 0.49 for global instructions), signifying that the baselines do not fully learn to avoid the puddle states. 

% Following Schaul et al. \shortcite{schaul2015universal}, we also evaluted our model in terms of policy quality, defined as the expected discounted reward achieved by following the softmax policy of the value predictions averaged over all maps in the test set, all instructions for a given map, and all start state for a given map-instruction pair. In practice, calculating policy quality amounts to running Value Iteration using the softmax of the predicted values as the transition probabilities. Policy quality is normalized such that an optimal policy has a score of 1 and a uniform random policy has a score of 0. Our model outperforms both baselines on this metric as well, although we do note that the performance of the baselines flip with respect to each other (\ref{tbl:rl_eval}). While the UVFA variant performed better on the train maps, it does not generalize to new environments as well as the CNN + LSTM. 

% Finally, given the nature of our environments, we can use the predicted value maps to infer a goal location by taking the position of the maximum. We use the Manhattan distance from this predicted position to the actual goal location as a third metric. The precision of our model's goal predictions is more than twice that of the baselines on local references and roughly $45\%$ better on global references. 



















